Direct Feedback Policy Optimization for AI Coding Agents

AI coding agents generate, modify, and validate code through multi-turn interactions. Existing reinforcement learning methods often rely on sparse terminal rewards, making it difficult to assess how intermediate decisions affect task outcomes, and group-relative methods also require repeated sampling for each task. We propose Direct Feedback Policy Optimization (DFPO), a single-trajectory reinforcement learning algorithm that trains directly from a single trajectory. DFPO achieves higher task resolution rates than GSPO under matched base models and execution harnesses.

==> dfpo-bibliography.tex <==
\makeatletter
\ExplSyntaxOn
\prop_new:N \g_dfpo_main_citations_prop
\bool_new:N \g_dfpo_in_appendix_bool
\seq_new:N \l_dfpo_bibitems_seq
\tl_new:N \g_dfpo_bibliography_tl
\cs_new_eq:NN \dfpo_natbib_sort_cites:n \NAT@sort@cites
\cs_new_eq:NN \dfpo_bibliography_begin:n \thebibliography
\cs_new_eq:NN \dfpo_bibliography_end: \endthebibliography

\cs_set_protected:Npn \NAT@sort@cites #1
  {
    \dfpo_natbib_sort_cites:n {#1}
    \bool_if:NF \g_dfpo_in_appendix_bool
      {
        \clist_map_inline:Nn \NAT@cite@list
          { \prop_gput:Nnn \g_dfpo_main_citations_prop {##1} {} }
      }
  }
\AddToHook{cmd/appendix/before}{\bool_gset_true:N \g_dfpo_in_appendix_bool}

\cs_new_protected:Npn \dfpo_print_bibitem:w [#1]#2#3\q_stop
  {
    \prop_if_in:NnTF \g_dfpo_main_citations_prop {#2}
      { \bool_if:NF \g_dfpo_in_appendix_bool { \bibitem[#1]{#2}#3 } }
      { \bool_if:NT \g_dfpo_in_appendix_bool { \bibitem[#1]{#2}#3 } }
  }

\RenewDocumentEnvironment {thebibliography} {m +b}
  {
    \bool_if:NF \g_dfpo_in_appendix_bool
      {
        \tl_gset:Nn \g_dfpo_bibliography_tl
          { \begin{thebibliography}{#1}#2\end{thebibliography} }
      }
    \seq_set_split:Nnn \l_dfpo_bibitems_seq {\bibitem} {#2}
    \seq_pop_left:NN \l_dfpo_bibitems_seq \l_tmpa_tl
    \dfpo_bibliography_begin:n {#1}
    \tl_use:N \l_tmpa_tl
    \seq_map_inline:Nn \l_dfpo_bibitems_seq { \dfpo_print_bibitem:w ##1\q_stop }
  }
  { \dfpo_bibliography_end: }

\NewDocumentCommand \DFPOAppendixBibliography {m}
  {
    \group_begin:
    \renewcommand{\refname}{#1}
    \setlength{\emergencystretch}{1em}
    \tl_use:N \g_dfpo_bibliography_tl
    \group_end:
  }
\ExplSyntaxOff
\makeatother

